Multi-Agent Coverage Control with Transient Behavior Consideration

This paper studies the multi-agent coverage control (MAC) problem where agents must dynamically learn an unknown density function while performing coverage tasks. Unlike many current theoretical frameworks that concentrate solely on the regret occurring at specific targeted sensory locations, our approach additionally considers the regret caused by transient behavior - the path from one location and another. We propose the multi-agent coverage control with the doubling trick (MAC-DT) algorithm and demonstrate that it achieves (approximated) regret of $\widetilde{O}(\sqrt{T})$ even when accounting for the transient behavior. Our result is also supported by numerical experiments, showcasing that the proposed algorithm manages to match or even outperform the baseline algorithms in simulation environments. We also show how our algorithm can be modified to handle safety constraints and further implement the algorithm on a real-robotic testbed.

==> Sections/Apdx-bound-destination-switch.tex <==
\section{Proof of Lemma \ref{lemma:destination-switch}}\label{apdx:destination-switch}

\begin{proof}%[Proof of Lemma \ref{lemma:destination-switch}]
The destination switch term is relatively easy to bound. When the agents haven't reached the destination, $\alpha\|w(s^\star)\|_1- \|w_{\UCB}^{(e)}(s_t)\|_1 \le \alpha\|w(s^\star)\|_1\le \alpha n\K$. When the agents have reached the destination, we have that $s_t = s_{dest} = \Oracle(w_{\UCB}^{(e)})$, and thus $\|w_{\UCB}^{(e)}(s_t)\|_1 \ge \alpha \max_{s}\|w_{\UCB}^{(e)}(s)\|_1 \ge \alpha \|w(s^\star)\|_1 $. Since the diameter of graph $G$ is $D$, it takes the agents at least $D$ steps to reach the destination, thus then for each episode, we have that $\sum_{t=t_e}^{t=t_{e+1}-1}[\|w(s^\star)\|_1- \|w_{\UCB}^{(e)}(s_t)\|_1] \le nD\K$. Then from Lemma \ref{lemma:bound-episode-number} in Appendix \ref{apdx:auxiliaries}, the number of episode $E$ can be bounded by  $E \le |V|\log(t_{E+1}-1) + 1$, the destination switch can then be bounded by ~$\bE \alpha nD\K E \le\alpha nD\K|V|(\log(t_{E+1}-1)+1)$.
\end{proof}

% \begin{lemma}[Bounding the Episode length]\label{lemma:bound-episode-number}
%     \begin{equation*}
%         E \le |V|\log(t_{E+1}-1) + 1
%     \end{equation*}
% \begin{proof}
%     The proof of Lemma \ref{lemma:bound-episode-number} is similar to the proof in \citep{zhang2023multi}, which is omitted for now.
% \end{proof}
% \end{lemma}


==> Sections/future_works_next_steps.tex <==
\section{Next Step and Potentially interesting questions:}
Next step: Finish the regret analysis first (also read the proofs in \cite{prajapat2022near}). One important question: Is doubling trick in really making a difference? (Without the doubling trick in line 5 of Algorithm \ref{alg:main}, our algorithm is basically just MaCOPT in \cite{prajapat2022near} + path planning, which doesn't really sound that interesting)\\

\noindent Potentially interesting questions:
\begin{enumerate}
    \item When the sensing area is smaller than the coverage area, could we find some counter-examples that the algorithm would fail?
    \item  A distributed version of the algorithm.
    \item Extension to the continuous setting (The doubling trick won't work for continuous setting without discretization. Is there other way to do this?)
    \item Generalize the the stochastic setting, will everything carry over (I think so, need two weeks to rigourously prove it)
\end{enumerate}




